Integrality properties in the Moduli Space of Elliptic Curves: Isogeny Case

For a fixed $j$-invariant $j_0$ of an elliptic curve without complex multiplication we bound the number of $j$-invariants $j$ that are algebraic units and such that elliptic curves corresponding to $j$ and $j_0$ are isogenous. Our bounds are effective. We also modify the problem slightly by fixing a singular modulus $\alpha$ and looking at all $j$ such that $j-\alpha$ is an algebraic unit and such that elliptic curves corresponding to $j$ and $j_0$ are isogenous. The number of such $j$ can again be bounded effectively.

==> noncm_ja_bound.tex <==

	With the same assumptions as in Proposition \ref{prop:noncm_N_bound}, if the elliptic curve corresponding to $j_0$ is
	isogenous to the elliptic curve corresponding to $j$, then the degree of the minimal isogeny is bounded by
	\begin{displaymath}
		\max\left\{10^{180}(Bc_1)^{20}, e^{Bc_1+Bc_2+c_3}, e^{\sqrt{45[\GL_2(\hat\Z):\rho_\infty(G_K)] + S +  12}},
									10^7 D(\tau_0^\sigma)^{18} X; \sigma\colon K \hookrightarrow \C\right\},
	\end{displaymath}
	where $B = 4C\cdot [\GL_2(\hat\Z):\rho_\infty(G_K)]\cdot[\Q(\alpha):\Q]/[K:\Q]$,
	$S$ is the constant from Proposition \ref{prop:j-a_N_bound}
	and $c_3 = 20 - h(j_0) + 6 \log(1+h(j_0))$.


